Dynamic Type Inference for Gradual Hindley--Milner Typing

Garcia and Cimini study a type inference problem for the ITGL, an implicitly and gradually typed language with let-polymorphism, and develop a sound and complete inference algorithm for it. Soundness and completeness mean that, if the algorithm succeeds, the input term can be translated to a well-typed term of an explicitly typed blame calculus by cast insertion and vice versa. However, in general, there are many possible translations depending on how type variables that were left undecided by static type inference are instantiated with concrete static types. Worse, the translated terms may behave differently---some evaluate to values but others raise blame. In this paper, we propose and formalize a new blame calculus $\lambda^{\textsf{DTI}}_{\textsf{B}}$ that avoids such divergence as an intermediate language for the ITGL. A main idea is to allow a term to contain type variables (that have not been instantiated during static type inference) and defer instantiation of these type variables to run time. We introduce dynamic type inference (DTI) into the semantics of $\lambda^{\textsf{DTI}}_{\textsf{B}}$ so that type variables are instantiated along reduction. The DTI-based semantics not only avoids the divergence described above but also is sound and complete with respect to the semantics of fully instantiated terms in the following sense: if the evaluation of a term succeeds (i.e., terminates with a value) in the DTI-based semantics, then there is a fully instantiated version of the term that also succeeds in the explicitly typed blame calculus and vice versa. Finally, we prove the gradual guarantee, which is an important correctness criterion of a gradually typed language, for the ITGL.

==> figures/def_ITGL_typed_term_precision.tex <==
\vspacerules

\begin{flushleft}
 \textbf{Typed Term Precision: }\fbox{$ \langle  \Gamma   \vdash   e  :  \ottnt{U} 
                 \sqsubseteq _{ S }  \ottnt{U'}  :  e'  \dashv  \Gamma'  \rangle $}
\end{flushleft}
\begin{center}
 $\ottdruleITPXXVarP{}$
 \vspacerule

 $\ottdruleITPXXConst{}$
 \vspacerule

 $\ottdruleITPXXOp{}$
 \vspacerule

 $\ottdruleITPXXAbsI{}$
 \vspacerule

 $\ottdruleITPXXAbsIE{}$
 \vspacerule

 $\ottdruleITPXXAbsEI{}$
 \vspacerule

 $\ottdruleITPXXAbsE{}$
 \vspacerule

 $\ottdruleITPXXApp{}$
 \vspacerule

 $\ottdruleITPXXLetP{}$
\end{center}


==> figures/def_cast_insertion.tex <==
% \begin{figure}[h]
  \begin{flushleft}
\textbf{Matching:} \fbox{$\ottnt{U}  \triangleright  \ottnt{U}$}
  \end{flushleft}
  \begin{center}
    $\ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}  \triangleright  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}$\qquad $\star  \triangleright  \star  \!\rightarrow\!  \star$
  \end{center}
  \vspacerules

  \begin{flushleft}
\textbf{Cast insertion rules:}  \fbox{$\Gamma  \vdash  e  \rightsquigarrow  \ottnt{f}  \ottsym{:}  \ottnt{U}$}
  \end{flushleft}
  \begin{center}
    $\ottdruleCIXXVarP{}$
    \vspacerule

    $\ottdruleCIXXConst{}$
    \vspacerule

    $\ottdruleCIXXAbsE{}$
    \vspacerule

    $\ottdruleCIXXAbsI{}$
    \vspacerule

    $\ottdruleCIXXApp{}$
    \vspacerule

    $\ottdruleCIXXLetP{}$
  \end{center}

%   \caption{Cast insertion rules from the ITGL to $\lambdaRTI$.}
%   \label{fig:def_cast_insertion}
% \end{figure}


==> proofs/gg.tex <==
% vim: spell
\begin{lemma} \label{lem:term_prec_to_type_prec}
  If $ \langle  \Gamma   \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S }  \ottnt{U'}  :  f'  \dashv  \Gamma'  \rangle $,
  then $ \ottnt{U}   \sqsubseteq _{ S }  \ottnt{U'} $.
\end{lemma}

\begin{proof}
  By induction on the term precision derivation.
\end{proof}

\begin{lemma} \label{lem:term_prec_to_typing}
  If $ \langle  \Gamma   \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S }  \ottnt{U'}  :  f'  \dashv  \Gamma'  \rangle $,
  then $\Gamma  \vdash  f  \ottsym{:}  \ottnt{U}$ and $\Gamma'  \vdash  f'  \ottsym{:}  \ottnt{U'}$.
\end{lemma}

\begin{proof}
  By induction on the term precision derivation.
\end{proof}

\begin{lemma} \label{lem:type_prec_right_var_equal}
  If $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S }  \ottmv{X} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S }  \ottmv{X} $,
  then $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{U_{{\mathrm{2}}}}$.
\end{lemma}

\begin{proof}
  By case analysis on the type precision rule applied last.
\end{proof}

\begin{lemma} \label{lem:prec_ground_contra}
  For any $S$, $w$, $w'$, $\ell$, and $\ottnt{U}$,
  there is no $\ottnt{G'_{{\mathrm{1}}}}$ and $\ottnt{G'_{{\mathrm{2}}}}$
  such that $ \ottnt{U}   \sqsubseteq _{ S }  \ottnt{G'_{{\mathrm{1}}}} $,
  $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{ S }  \star  :  w'  \ottsym{:}   \ottnt{G'_{{\mathrm{2}}}} \Rightarrow  \unskip ^ { \ell }  \! \star   \dashv   \emptyset   \rangle $,
  and $\ottnt{G'_{{\mathrm{1}}}}  \neq  \ottnt{G'_{{\mathrm{2}}}}$.
\end{lemma}

\begin{proof}
  By induction on the term precision derivation.
\end{proof}

% \subsection{Substitution}

\ifrestate
\lemLeftSubstPreservePrec*
\else
\begin{lemma} \label{lem:left_subst_preserve_prec}
  For any $S$.
  \begin{enumerate}
    \item
      If $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $,
      then $ S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
    \item
      If $ \langle   \emptyset    \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $,
      then $ \langle   \emptyset    \vdash   S  \ottsym{(}  f  \ottsym{)}  :  S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $.
  \end{enumerate}
\end{lemma}
\fi

\begin{proof}
  \leavevmode
  \begin{enumerate}
    \item By induction on the derivation of $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
      \begin{caseanalysis}
        \case{\rnp{P\_TyVar}}
        We are given $ \ottnt{T}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottmv{X'} $ for some $\ottnt{T}$ and $\ottmv{X'}$.
        By inversion, $S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \ottnt{T}$.
        By definition, $ S  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X'}  \ottsym{)} = S  \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{)} = S  \ottsym{(}  \ottnt{T}  \ottsym{)}$.
        By \rnp{P\_TyVar}, $ S  \ottsym{(}  \ottnt{T}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottmv{X'} $.

        \otherwise Obvious.
      \end{caseanalysis}

    \item By induction on the derivation of $ \langle  \Gamma   \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv  \Gamma'  \rangle $ using Lemma \ref{lem:left_subst_preserve_prec}.1.
      \qedhere
  \end{enumerate}
\end{proof}

\ifrestate
\lemRightSubstPreservePrec*
\else
\begin{lemma} \label{lem:right_subst_preserve_prec}
  Suppose $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
  \begin{enumerate}
    \item
      If $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $,
      then $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)} $.
    \item
      If $ \langle   \emptyset    \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $,
      then $ \langle   \emptyset    \vdash   f  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  S'  \ottsym{(}  f'  \ottsym{)}  \dashv   \emptyset   \rangle $.
  \end{enumerate}
\end{lemma}
\fi % ifrestate

\begin{proof}
  \leavevmode
  \begin{enumerate}
    \item By induction on the derivation of $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
      \begin{caseanalysis}
        \case{\rnp{P\_TyVar}}
        We are given $ \ottnt{T}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottmv{X'} $ for some $\ottnt{T}$ and $\ottmv{X'}$.
        By inversion, $S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \ottnt{T}$.
        Obviously, $\ottmv{X'} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}$.
        So, $ S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  S'  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{)} =   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'   \ottsym{(}  \ottmv{X'}  \ottsym{)} = S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)} = \ottnt{T}$.
        By \rnp{P\_TyVar}, $ \ottnt{T}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottmv{X'}  \ottsym{)} $.

        \otherwise Obvious.
      \end{caseanalysis}

    \item By induction on the derivation of $ \langle  \Gamma   \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv  \Gamma'  \rangle $
      \qedhere
  \end{enumerate}
\end{proof}

% \subsection{Inversion}

\begin{lemma} \label{lem:term_prec_inversion1}
  If $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \star  :  w'  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell' }  \! \star   \dashv   \emptyset   \rangle $
  and $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{G'} $,
  then $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{G'}  :  w'  \dashv   \emptyset   \rangle $,
\end{lemma}

\begin{proof}
  By induction on the term precision derivation.
\end{proof}

\begin{lemma} \label{lem:term_prec_inversion3}
  If $ \langle   \emptyset    \vdash   f  \ottsym{:}   \ottnt{U} \Rightarrow  \unskip ^ { \ell }  \! \star   :  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $
  then $ \langle   \emptyset    \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $,
\end{lemma}

\begin{proof}
  By induction on the term precision derivation.
\end{proof}

\begin{lemma} \label{lem:term_prec_inversion4}
  If $ \langle   \emptyset    \vdash   w  :  \iota   \sqsubseteq _{ S_{{\mathrm{0}}} }  \iota  :  w'  \dashv   \emptyset   \rangle $,
  then there exists $\ottnt{c}$ such that $w  \ottsym{=}  w' = c$.
\end{lemma}

\begin{proof}
  By induction on the term precision derivation.
\end{proof}

% \subsection{Simulation}

\ifrestate
\lemPrecCatchUpLeftValue*
\else
\begin{lemma}[Catchup to Value on the Left] \label{lem:prec_catch_up_left_value}
  If $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $,
  then there exists $S'$, $S'_{{\mathrm{0}}}$, and $w'$
  such that $f' \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'$,
  $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  w'  \dashv   \emptyset   \rangle $,
  and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
\end{lemma}
\fi %ifrestate

\begin{proof}
  By induction on the term precision derivation.

  \begin{caseanalysis}
    \case{\rnp{P\_Const} and \rnp{P\_Abs}}
    Obvious.

    \case{\rnp{P\_Cast}}
    We are given,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}   :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}   \dashv   \emptyset   \rangle $,
    where $w  \ottsym{=}  w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U} $ and $f'  \ottsym{=}  f'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'} $
    for some $w_{{\mathrm{1}}}$, $f'_{{\mathrm{1}}}$, $\ottnt{U_{{\mathrm{1}}}}$ and $\ottnt{U'_{{\mathrm{1}}}}$.
    By inversion,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $,
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $, $\ottnt{U_{{\mathrm{1}}}}  \sim  \ottnt{U}$, and $\ottnt{U'_{{\mathrm{1}}}}  \sim  \ottnt{U'}$.
    %
    By the IH, there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{1}}}$ and $w'_{{\mathrm{1}}}$ such that
    $f'_{{\mathrm{1}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{1}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{1}}}$,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{1}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    %
    By case analysis on $\ottnt{U'_{{\mathrm{1}}}}  \sim  \ottnt{U'}$.

    \begin{caseanalysis}
      \case{$\iota  \sim  \iota$ for some $\iota$}
      Here, $w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U} $ is a value and $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \iota $.
      By Lemma \ref{lem:canonical_forms},
      $\ottnt{U}$ is a function type or the dynamic type.
      Contradiction.

      \case{$\ottmv{X'}  \sim  \ottmv{X'}$ for some $\ottmv{X'}$}
      By case analysis on $S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}$.
      \begin{caseanalysis}
        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \iota$}
        Similarly to the case $\iota  \sim  \iota$.

        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \ottmv{X''}$ for some $\ottmv{X''}$}
        By Lemma \ref{lem:term_prec_to_typing}, $ \emptyset   \vdash  w'_{{\mathrm{1}}}  \ottsym{:}  \ottmv{X''}$.
        This contradicts Lemma \ref{lem:canonical_forms}.

        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}$ is a function type}
        By Lemma \ref{lem:type_prec_right_var_equal}, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{U}$.
        By Lemma \ref{lem:term_prec_to_type_prec},
        $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $.
        So, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $.
        We finish by \rnp{P\_Cast}.
      \end{caseanalysis}

      \case{$\star  \sim  \star$}
      By \rnp{R\_IdStar}, $w'_{{\mathrm{1}}}  \ottsym{:}   S'_{{\mathrm{1}}}  \ottsym{(}  \star  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{1}}}  \ottsym{(}  \star  \ottsym{)}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{1}}}$.
      By definition, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star $.
      We finish by \rnp{P\_CastL}.

      \case{$\star  \sim  \ottnt{U'}$ where $\ottnt{U'}  \neq  \star$}
      Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \star  \ottsym{)}  \ottsym{=}  \star$.
      By Lemma \ref{lem:canonical_forms},
      there exist $w'_{{\mathrm{11}}}$ and $\ottnt{G'}$ such that $w'_{{\mathrm{1}}}  \ottsym{=}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \! \star $.
      By case analysis on $\ottnt{U'}$.

      \begin{caseanalysis}
        \case{$\ottnt{U'}  \ottsym{=}  \iota$ for some $\iota$}
        Here, $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \iota $.
        By Lemma \ref{lem:canonical_forms},
        $\ottnt{U}$ is a function type or the dynamic type.
        Contradiction.

        \case{$\ottnt{U'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
        Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \star  \!\rightarrow\!  \star  \ottsym{)}  \ottsym{=}  \star  \!\rightarrow\!  \star$.
        By Lemma \ref{lem:term_prec_to_type_prec}, $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \star  \!\rightarrow\!  \star $.
        By definition, $\ottnt{U}$ is a function type.
        By Lemma \ref{lem:canonical_forms}, $\ottnt{U_{{\mathrm{1}}}}$ is also a function type.
        So, by definition, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
        %
        By case analysis on $\ottnt{G'}$.

        \begin{caseanalysis}
          \case{$\ottnt{G'}  \ottsym{=}  \iota$ for some $\iota$}
          We are given,
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  :  w'_{{\mathrm{11}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \! \star   \dashv   \emptyset   \rangle $.
          This contradicts Lemma \ref{lem:prec_ground_contra}.

          \case{$\ottnt{G'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
          By \rnp{R\_Succeed}, $w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! \star  \!\rightarrow\!  \star   \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{11}}}$.
          By Lemma \ref{lem:term_prec_inversion1},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.
          We finish by \rnp{P\_CastL}.
        \end{caseanalysis}

        \case{$\ottnt{U'}  \ottsym{=}  \ottmv{X'}$ for some $\ottmv{X'}$}
        If $S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}$ is not a type variable,
        then similarly to the other cases.

        % FIXME: Add explanation.
        % Because generated subst does not contain a subst like {X':->X'}
        Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \ottmv{X'}$ because $S'_{{\mathrm{1}}}$ is generated by DTI.
        By case analysis on $\ottnt{G'}$.
        \begin{caseanalysis}
          \case{$\ottnt{G'}  \ottsym{=}  \iota$ for some $\iota$}
          By Lemma \ref{lem:term_prec_to_type_prec},
          $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottmv{X'} $.
          %
          By Lemma \ref{lem:canonical_forms},
          $\ottnt{U}$ is the dynamic type or a function type.
          By case analysis on $\ottnt{U}$.
          \begin{caseanalysis}
            \case{$\ottnt{U}$ is the dynamic type}
            Contradiction.

            \case{$\ottnt{U}$ is a function type}
            By Lemma \ref{lem:canonical_forms},
            $\ottnt{U_{{\mathrm{1}}}}$ is also a function type.
            By definition, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
            This contradicts Lemma \ref{lem:prec_ground_contra}.
          \end{caseanalysis}

          \case{$\ottnt{G'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
          We are given, $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  :  w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \! \star   \dashv   \emptyset   \rangle $.
          %
          % TODO: We may state the following as a lemma
          By Lemma \ref{lem:term_prec_to_type_prec},
          $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottmv{X'} $.
          By Lemma \ref{lem:canonical_forms},
          $\ottnt{U}$ is the dynamic type or a function type.
          If $\ottnt{U}$ is the dynamic type, then contradictory.
          So, $\ottnt{U}$ is a function type and
          there exist $\ottnt{T_{{\mathrm{1}}}}$ and $\ottnt{T_{{\mathrm{2}}}}$ such that $\ottnt{U}  \ottsym{=}  \ottnt{T_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{T_{{\mathrm{2}}}}$.
          By Lemma \ref{lem:canonical_forms}, $\ottnt{U_{{\mathrm{1}}}}$ is also a function type.
          By definition, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.

          By \rnp{R\_InstArrow} and \rnp{R\_Succeed},
          $w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! \ottmv{X'}   \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell' }  \! \ottmv{X'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X'_{{\mathrm{2}}}} $
          where $S'_{{\mathrm{2}}}  \ottsym{=}  [  \ottmv{X'}  :=  \ottmv{X'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X'_{{\mathrm{2}}}}  ]$ and $\ottmv{X'_{{\mathrm{1}}}}$ and $\ottmv{X'_{{\mathrm{2}}}}$ are fresh.

          By Lemma \ref{lem:term_prec_inversion1},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $.
          So, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \ottmv{X'} $.

          Here, $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{3}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $
          and $ \ottnt{U}   \sqsubseteq _{   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $
          where $S'_{{\mathrm{3}}}  \ottsym{=}  [  \ottmv{X'_{{\mathrm{1}}}}  :=  \ottnt{T_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{X'_{{\mathrm{2}}}}  :=  \ottnt{T_{{\mathrm{2}}}}  ]$.
          %
          We finish by \rnp{P\_Cast}.
        \end{caseanalysis}

        \case{$\ottnt{U'}  \ottsym{=}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}$ for some $\ottnt{U'_{{\mathrm{11}}}}$ and $\ottnt{U'_{{\mathrm{12}}}}$ where $\ottnt{U'}  \neq  \star  \!\rightarrow\!  \star$}
        \leavevmode\\
        By Lemma \ref{lem:term_prec_to_type_prec}, $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} $.
        By definition, $\ottnt{U}$ is a function type.
        By Lemma \ref{lem:canonical_forms}, $\ottnt{U_{{\mathrm{1}}}}$ is a function type.
        By definition, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
        By case analysis on $\ottnt{G'}$.

        \begin{caseanalysis}
          \case{$\ottnt{G'}  \ottsym{=}  \iota$ for some $\iota$}
          We are given,
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  :  w'_{{\mathrm{11}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \! \star   \dashv   \emptyset   \rangle $.
          This contradicts Lemma \ref{lem:prec_ground_contra}.

          \case{$\ottnt{G'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
          We are given,
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  :  w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \! \star   \dashv   \emptyset   \rangle $.
          By definition,
          $w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}   \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} $.
          %
          By Lemma \ref{lem:term_prec_inversion1},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
          %
          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} $.
          %
          We finish by \rnp{P\_Cast}.
        \end{caseanalysis}
      \end{caseanalysis}

      \case{$\ottnt{U'_{{\mathrm{1}}}}  \sim  \star$ where $\ottnt{U'_{{\mathrm{1}}}}  \neq  \star$}
      By case analysis on $\ottnt{U'_{{\mathrm{1}}}}$.

      \begin{caseanalysis}
        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}$ is a ground type}
        % Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}$ is also a ground type.
        Obvious.

        \otherwise
        There exist $\ottnt{U'_{{\mathrm{11}}}}$ and $\ottnt{U'_{{\mathrm{12}}}}$ such that $S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  \ottsym{=}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}$.
        Here,
        $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.
        By Lemma \ref{lem:term_prec_to_type_prec},
        $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)} $.
        By definition, $\ottnt{U_{{\mathrm{1}}}}$ is a function type.
        By Lemma \ref{lem:canonical_forms},
        $\ottnt{U}$ is the dynamic type or a function type.
        By case analysis on $\ottnt{U}$.

        \begin{caseanalysis}
          \case{$\ottnt{U}  \ottsym{=}  \star$}
          By Lemma \ref{lem:canonical_forms}, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star  \!\rightarrow\!  \star$.
          Here, $ \star  \!\rightarrow\!  \star   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)} $
          and $S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}$ is not a ground type.
          Contradiction.

          \case{$\ottnt{U}$ is a function type}
          By \rnp{R\_Ground},
          $w'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \star  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell' }  \! \star  $.
          We finish by \rnp{P\_CastR} and \rnp{P\_Cast}.
        \end{caseanalysis}
      \end{caseanalysis}

      \case{$\ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \sim  \ottnt{U'_{{\mathrm{13}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{14}}}}$ for some $\ottnt{U'_{{\mathrm{11}}}}$, $\ottnt{U'_{{\mathrm{12}}}}$, $\ottnt{U'_{{\mathrm{13}}}}$, and $\ottnt{U'_{{\mathrm{14}}}}$}
      Obvious.
    \end{caseanalysis}

    \case{\rnp{P\_CastL}}
    Here, $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}   :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $,
    where $w  \ottsym{=}  w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U} $ for some $w_{{\mathrm{1}}}$ and $\ottnt{U_{{\mathrm{1}}}}$.
    By inversion, $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $,
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $, $\ottnt{U_{{\mathrm{1}}}}  \sim  \ottnt{U}$.
    By the IH, there exist $S'_{{\mathrm{0}}}$, $S'$, and $w'$ such that
    $f' \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'$,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  w'  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    By Lemma \ref{lem:term_prec_to_type_prec},
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
    By Lemma \ref{lem:right_subst_preserve_prec},
    $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)} $.
    We finish by \rnp{P\_CastL}.

    \case{\rnp{P\_CastR}}
    Here, $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}   \dashv   \emptyset   \rangle $,
    where $f'  \ottsym{=}  f'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'} $ for some $f'_{{\mathrm{1}}}$ and $\ottnt{U'_{{\mathrm{1}}}}$.
    By inversion,
    $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $,
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $, and $\ottnt{U'_{{\mathrm{1}}}}  \sim  \ottnt{U'}$.
    %
    By the IH, there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{1}}}$ and $w'_{{\mathrm{1}}}$ such that
    $f'_{{\mathrm{1}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{1}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{1}}}$,
    $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{1}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    %
    By case analysis on $\ottnt{U'_{{\mathrm{1}}}}  \sim  \ottnt{U'}$.

    \begin{caseanalysis}
      \case{$\iota  \sim  \iota$ for some $\iota$}
      Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \iota  \ottsym{)}  \ottsym{=}  \iota$.
      By definition, $w'_{{\mathrm{1}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell' }  \! \iota  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{1}}}$.
      Obvious.

      \case{$\ottmv{X'}  \sim  \ottmv{X'}$ for some $\ottmv{X'}$}
      By case analysis on $S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}$.
      \begin{caseanalysis}
        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \iota$}
        Similarly to the case $\iota  \sim  \iota$.

        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \ottmv{X''}$ for some $\ottmv{X''}$}
        By Lemma \ref{lem:term_prec_to_typing}, $ \emptyset   \vdash  w'_{{\mathrm{1}}}  \ottsym{:}  \ottmv{X''}$.
        This contradicts Lemma \ref{lem:canonical_forms}.

        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}$ is a function type}
        By Lemma \ref{lem:term_prec_to_type_prec},
        $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $.
        We finish by \rnp{P\_CastR}.
      \end{caseanalysis}

      \case{$\star  \sim  \star$}
      Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \star  \ottsym{)}  \ottsym{=}  \star$.
      By \rnp{R\_IdStar}, $w'_{{\mathrm{1}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell' }  \! \star  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{1}}}$.
      Obvious.

      \case{$\star  \sim  \ottnt{U'}$ where $\ottnt{U'}  \neq  \star$}
      Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \star  \ottsym{)}  \ottsym{=}  \star$.
      By Lemma \ref{lem:canonical_forms},
      there exist $w'_{{\mathrm{11}}}$ and $\ottnt{G'}$ such that $w'_{{\mathrm{1}}}  \ottsym{=}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \! \star $.
      By case analysis on $\ottnt{U'}$.

      \begin{caseanalysis}
        \case{$\ottnt{U'}  \ottsym{=}  \iota$ for some $\iota$}
        By case analysis on $\ottnt{G'}$.
        \begin{caseanalysis}
          \case{$\ottnt{G'}  \ottsym{=}  \iota$}
          By \rnp{R\_Succeed}, $w'_{{\mathrm{11}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! \iota   \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{11}}}$.
          By Lemma \ref{lem:term_prec_inversion1},
          $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \iota  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.

          \case{$\ottnt{G'}  \neq  \iota$}
          This contradicts Lemma \ref{lem:prec_ground_contra}.
        \end{caseanalysis}

        \case{$\ottnt{U'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
        By case analysis on $\ottnt{G'}$.
        \begin{caseanalysis}
          \case{$\ottnt{G'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
          By \rnp{R\_Succeed}, $w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! \star  \!\rightarrow\!  \star   \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{11}}}$.
          By Lemma \ref{lem:term_prec_inversion1},
          $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.

          \case{$\ottnt{G'}  \neq  \star  \!\rightarrow\!  \star$}
          This contradicts Lemma \ref{lem:prec_ground_contra}.
        \end{caseanalysis}

        \case{$\ottnt{U'}  \ottsym{=}  \ottmv{X'}$ for some $\ottmv{X'}$}
        If $S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}$ is not a type variable,
        then similarly to the other cases.

        % FIXME: Add explanation.
        % Because generated subst does not contain a subst like {X':->X'}
        Here, $S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)}  \ottsym{=}  \ottmv{X'}$ because $S'_{{\mathrm{1}}}$ is generated by DTI.
        By case analysis on $\ottnt{G'}$.
        \begin{caseanalysis}
          \case{$\ottnt{G'}  \ottsym{=}  \iota$ for some $\iota$}
          By case analysis on $\ottnt{U}$ using Lemma \ref{lem:canonical_forms}.

          \begin{caseanalysis}
            \case{$\ottnt{U}  \ottsym{=}  \iota$}
            By definition, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \iota $.
            By Lemma \ref{lem:term_prec_inversion1},
            $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \iota  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.

            By \rnp{R\_InstBase}, $w'_{{\mathrm{11}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! \ottmv{X'}   \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }  \, S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}$
            where $S'_{{\mathrm{2}}}  \ottsym{=}  [  \ottmv{X'}  :=  \iota  ]$.

            By Lemma \ref{lem:right_subst_preserve_prec},
            $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \iota  :  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.

            \case{$\ottnt{U}  \ottsym{=}  \ottnt{G}$ where $\ottnt{G}  \neq  \ottnt{G'}$}
            This contradicts Lemma \ref{lem:prec_ground_contra}.

            \case{$\ottnt{U}$ is a function type}
            By definition, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
            This contradicts Lemma \ref{lem:prec_ground_contra}.
          \end{caseanalysis}

          \case{$\ottnt{G'}  \ottsym{=}  \star  \!\rightarrow\!  \star$}
          By Lemma \ref{lem:canonical_forms},
          $\ottnt{U}$ is a ground type, the dynamic type, or a function type.
          By case analysis on $\ottnt{U}$.

          \begin{caseanalysis}
            \case{$\ottnt{U}  \ottsym{=}  \ottnt{G}$ where $\ottnt{G}  \neq  \ottnt{G'}$}
            This contradicts Lemma \ref{lem:prec_ground_contra}.

            \case{$\ottnt{U}  \ottsym{=}  \star$}
            Contradiction.

            \case{$\ottnt{U}$ is a function type}
            By definition, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
            By Lemma \ref{lem:term_prec_inversion1},
            $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.

            By \rnp{R\_InstArrow}, $w'_{{\mathrm{11}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell'_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell' }  \! \ottmv{X'}   \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell' }  \! \ottmv{X'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X'_{{\mathrm{2}}}} $
            where $S'_{{\mathrm{2}}}  \ottsym{=}  [  \ottmv{X'}  :=  \ottmv{X'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X'_{{\mathrm{2}}}}  ]$.

            By Lemma \ref{lem:term_prec_to_type_prec},
            $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottmv{X'} $.
            By Lemma \ref{lem:right_subst_preserve_prec},
            $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $.
            So, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \ottmv{X'} $.
            Here, $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{3}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
            By Lemma \ref{lem:right_subst_preserve_prec},
            $ \langle   \emptyset    \vdash   w  :  \ottnt{U}   \sqsubseteq _{   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star  :  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $
            and $ \ottnt{U}   \sqsubseteq _{   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottmv{X'}  \ottsym{)} $
            where $S'_{{\mathrm{3}}}  \ottsym{=}  [  \ottmv{X'_{{\mathrm{1}}}}  :=  \ottnt{T_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{X'_{{\mathrm{2}}}}  :=  \ottnt{T_{{\mathrm{2}}}}  ]$.
            %
            We finish by \rnp{P\_CastR}.
          \end{caseanalysis}
        \end{caseanalysis}

        \case{$\ottnt{U'}  \ottsym{=}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}$ for some $\ottnt{U'_{{\mathrm{11}}}}$ and $\ottnt{U'_{{\mathrm{12}}}}$ where $\ottnt{U'}  \neq  \star  \!\rightarrow\!  \star$}
        \leavevmode\\
        By Lemma \ref{lem:term_prec_to_type_prec}, $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} $.
        By definition, $\ottnt{U}$ is a function type.
        So, by definition, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
        By Lemma \ref{lem:right_subst_preserve_prec},
        $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} $.

        By \rnp{R\_Expand},
        $w'_{{\mathrm{1}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{1}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell' }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}  $.
        We finish by \rnp{P\_CastR}.
      \end{caseanalysis}

      \case{$\ottnt{U'_{{\mathrm{1}}}}  \sim  \star$ where $\ottnt{U'_{{\mathrm{1}}}}  \neq  \star$}
      By case analysis on $\ottnt{U'_{{\mathrm{1}}}}$.

      \begin{caseanalysis}
        \case{$S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}$ is a ground type}
        Obvious.

        \otherwise
        There exist $\ottnt{U'_{{\mathrm{11}}}}$ and $\ottnt{U'_{{\mathrm{12}}}}$ such that $S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  \ottsym{=}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}$.
        By Lemma \ref{lem:term_prec_to_type_prec},
        $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{1}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)} $.
        By definition, $\ottnt{U}$ is a function type.
        So, $ \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \star  \!\rightarrow\!  \star $.
        By \rnp{R\_Ground},
        $w'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \star  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w'_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell' }  \! \star  $.
        We finish by \rnp{P\_CastR}.
      \end{caseanalysis}

      \case{$\ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \sim  \ottnt{U'_{{\mathrm{13}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{14}}}}$ for some $\ottnt{U'_{{\mathrm{11}}}}$, $\ottnt{U'_{{\mathrm{12}}}}$, $\ottnt{U'_{{\mathrm{13}}}}$, and $\ottnt{U'_{{\mathrm{14}}}}$}
      Obvious.
    \end{caseanalysis}

    \otherwise
    Cannot happen.  \qedhere
  \end{caseanalysis}
\end{proof}

\begin{lemma} \label{lem:subst_preserve_term_prec}
  If $ \langle   \Gamma ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}     \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \Gamma' ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}    \rangle $
  and $ \langle  \Gamma   \vdash   w  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  w'  \dashv  \Gamma'  \rangle $,
  then there exists $S'_{{\mathrm{0}}}$ such that
  $ \langle  \Gamma   \vdash   f  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w   ]  :  \ottnt{U}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'   ]  \dashv  \Gamma'  \rangle $
  and $\forall \, \ottmv{X} \, \in \, \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}  \ottsym{.}  S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}$.

\end{lemma}

\begin{proof}
  By induction on $ \langle   \Gamma ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}     \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \Gamma' ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}    \rangle $.

  \begin{caseanalysis}
    \case{\rnp{P\_VarP}}
    We are given
    $ \langle   \Gamma ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}     \vdash   \ottmv{x'}  [   \overrightarrow{ \ottnt{T_{\ottmv{i}}} }   ]  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  \ottmv{x'}  [   \overrightarrow{ \ottnt{T'_{\ottmv{i}}} }   ]  \dashv   \Gamma' ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}    \rangle $
    for some $\ottmv{x'}$, $ \overrightarrow{ \ottnt{T_{\ottmv{i}}} } $ and $ \overrightarrow{ \ottnt{T'_{\ottmv{i}}} } $.

    If $\ottmv{x}  \neq  \ottmv{x'}$, then obvious.
    Otherwise, we are given
    $ \langle   \Gamma ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}     \vdash   \ottmv{x}  [   \overrightarrow{ \ottnt{T_{\ottmv{i}}} }   ]  :  S  \ottsym{(}  \ottnt{U_{{\mathrm{1}}}}  \ottsym{)}   \sqsubseteq _{ S_{{\mathrm{0}}} }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  \ottmv{x}  [   \overrightarrow{ \ottnt{T'_{\ottmv{i}}} }   ]  \dashv   \Gamma' ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}    \rangle $,
    $S  \ottsym{(}  \ottnt{U_{{\mathrm{1}}}}  \ottsym{)}  \ottsym{=}  \ottnt{U}$, and $S  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  \ottsym{=}  \ottnt{U'}$
    where $S  \ottsym{=}  [   \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   :=   \overrightarrow{ \ottnt{T_{\ottmv{i}}} }   ]$ and $S'  \ottsym{=}  [   \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   :=   \overrightarrow{ \ottnt{T'_{\ottmv{i}}} }   ]$.

    By inversion,
    $\ottmv{x}  \ottsym{:}  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}} \, \in \,  \Gamma ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}  $,
    $\ottmv{x}  \ottsym{:}  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}} \, \in \,  \Gamma ,   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}  $,
    $ S  \ottsym{(}  \ottnt{U_{{\mathrm{1}}}}  \ottsym{)}   \sqsubseteq _{ S_{{\mathrm{0}}} }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)} $,
    $\exists \, S'_{{\mathrm{0}}}  \ottsym{.} \, \forall \, \ottmv{X} \, \in \, \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}  \ottsym{.}  S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}  \circ  S'   \ottsym{(}  \ottmv{X}  \ottsym{)}$, and
    $S_{{\mathrm{0}}}  \ottsym{(}   \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{)}  \ottsym{=}  S_{{\mathrm{0}}}  \ottsym{(}   \overrightarrow{ \ottnt{T'_{\ottmv{i}}} }   \ottsym{)}$.

    Here, $S_{{\mathrm{0}}}  \ottsym{(}   \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{)}  \ottsym{=}  S_{{\mathrm{0}}}  \ottsym{(}   \overrightarrow{ \ottnt{T'_{\ottmv{i}}} }   \ottsym{)}$.
    So, $\forall \, \ottmv{X} \, \in \, \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}  \ottsym{.}  S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}$.

    By Lemma \ref{lem:right_subst_preserve_prec},
    $ \langle  \Gamma   \vdash   w  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  S'  \ottsym{(}  w'  \ottsym{)}  \dashv  \Gamma'  \rangle $.

    By Lemma \ref{lem:left_subst_preserve_prec},
    $ \langle  \Gamma   \vdash   S  \ottsym{(}  w  \ottsym{)}  :  S  \ottsym{(}  \ottnt{U_{{\mathrm{1}}}}  \ottsym{)}   \sqsubseteq _{   S  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  S'  \ottsym{(}  w'  \ottsym{)}  \dashv  \Gamma'  \rangle $.

    Here, $\textit{dom} \, \ottsym{(}  S  \ottsym{)}  \cap  \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}  \ottsym{=}   \emptyset $.
    So, $\forall \, \ottmv{X} \, \in \, \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}  \ottsym{.}  S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S  \circ   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.

    \otherwise  Obvious.  \qedhere
  \end{caseanalysis}
\end{proof}

\ifrestate
\lemTermPrecSimulationApp*
\else
\begin{lemma}[Simulation of Function Application] \label{lem:term_prec_simulation_app}
  If $ \langle   \emptyset    \vdash    \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  f_{{\mathrm{1}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $
  and $ \langle   \emptyset    \vdash   w_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  w'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
  then there exists $S'_{{\mathrm{0}}}$, $S'$ and $f'$ such that
  $w'_{{\mathrm{1}}} \, w'_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^+ \hspace{0.2em}  \, f'$,
  $ \langle   \emptyset    \vdash   f_{{\mathrm{1}}}  [  \ottmv{x}  \ottsym{:=}  w_{{\mathrm{2}}}  ]  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  \ottnt{f'}  \dashv   \emptyset   \rangle $,
  and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
\end{lemma}
\fi %ifrestate

\begin{proof}
  By induction on $ \langle   \emptyset    \vdash    \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  f_{{\mathrm{1}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.

  \begin{caseanalysis}
    \case{\rnp{P\_Abs}}
    We are given
    $ \langle   \emptyset    \vdash    \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  f_{{\mathrm{1}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :   \lambda  \ottmv{x} \!:\!  \ottnt{U'_{{\mathrm{1}}}}  .\,  f'_{{\mathrm{1}}}   \dashv   \emptyset   \rangle $
    and $w'_{{\mathrm{1}}}  \ottsym{=}   \lambda  \ottmv{x} \!:\!  \ottnt{U'_{{\mathrm{1}}}}  .\,  f'_{{\mathrm{1}}} $ for some $f'_{{\mathrm{1}}}$.
    By inversion,
    $ \langle   \ottmv{x}  :  \ottnt{U_{{\mathrm{1}}}}    \vdash   f_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}}  :  f'_{{\mathrm{1}}}  \dashv   \ottmv{x}  :  \ottnt{U'_{{\mathrm{1}}}}   \rangle $
    and $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $.
    By \rnp{R\_Beta}, $\ottsym{(}   \lambda  \ottmv{x} \!:\!  \ottnt{U'_{{\mathrm{1}}}}  .\,  f'_{{\mathrm{1}}}   \ottsym{)} \, w'_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{1}}}  [  \ottmv{x}  \ottsym{:=}  w'_{{\mathrm{2}}}  ]$.
    By Lemma \ref{lem:subst_preserve_term_prec},
    $ \langle   \emptyset    \vdash   f_{{\mathrm{1}}}  [  \ottmv{x}  \ottsym{:=}  w_{{\mathrm{2}}}  ]  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}}  :  f'_{{\mathrm{1}}}  [  \ottmv{x}  \ottsym{:=}  w'_{{\mathrm{2}}}  ]  \dashv   \emptyset   \rangle $.

    \case{\rnp{P\_CastR}}
    By Lemma \ref{lem:canonical_forms},
    there exist $w'_{{\mathrm{11}}}$, $\ottnt{U'_{{\mathrm{11}}}}$, $\ottnt{U'_{{\mathrm{12}}}}$, and $\ell'$ such that
    $ \langle   \emptyset    \vdash    \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  f_{{\mathrm{1}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}   \dashv   \emptyset   \rangle $
    and $w'_{{\mathrm{1}}}  \ottsym{=}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.

    By inversion,
    $ \langle   \emptyset    \vdash    \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  f_{{\mathrm{1}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
    and $ \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}} $.
    By Lemma \ref{lem:term_prec_to_type_prec},
    $ \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{12}}}} $.

    By \rnp{R\_AppCast},
    $\ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}   \ottsym{)} \, w'_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \ottsym{(}  w'_{{\mathrm{11}}} \, \ottsym{(}  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{2}}}} $.

    By \rnp{P\_CastR},
    $ \langle   \emptyset    \vdash   w_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  :  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \dashv   \emptyset   \rangle $.

    By Lemma \ref{lem:prec_catch_up_left_value},
    there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{2}}}$, and $w''_{{\mathrm{2}}}$ such that
    $w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w''_{{\mathrm{2}}}$,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \ottsym{)}  :  w''_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    So,
    $\ottsym{(}  w'_{{\mathrm{11}}} \, \ottsym{(}  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{2}}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, \ottsym{(}  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w''_{{\mathrm{2}}}  \ottsym{)}  \ottsym{:}   S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $.

    By Lemma \ref{lem:right_subst_preserve_prec},
    $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $ and
    $ \langle   \emptyset    \vdash    \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  f_{{\mathrm{1}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}  :  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.

    By the IH, there exist $S''_{{\mathrm{0}}}$, $S'_{{\mathrm{3}}}$, and $f''$ such that
    $S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w''_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{3}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^+ \hspace{0.2em}  \, f''$,
    $ \langle   \emptyset    \vdash   f_{{\mathrm{1}}}  [  \ottmv{x}  \ottsym{:=}  w_{{\mathrm{2}}}  ]  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}  :  f''  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{3}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    By Lemma \ref{lem:right_subst_preserve_prec},
    $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $.

    So,
    $\ottsym{(}  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w''_{{\mathrm{2}}}  \ottsym{)}  \ottsym{:}   S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{3}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^+ \hspace{0.2em}  \, f''  \ottsym{:}    S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \!  S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ     S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{3}}}   \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    % FIXME: the above is little bit informal
    % but it seems to be OK
    % $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    % ==> $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   \ottsym{(}     S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{3}}}   \ottsym{)}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    We finish by \rnp{P\_CastR}.

    \otherwise Cannot happen.  \qedhere
  \end{caseanalysis}
\end{proof}

\ifrestate
\lemTermPrecSimulationUnwrap*
\else
\begin{lemma}[Simulation of Unwrapping] \label{lem:term_prec_simulation_unwrap}
  If $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $
  and $ \langle   \emptyset    \vdash   w_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  w'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
  then there exists $S'_{{\mathrm{0}}}$, $S'$, and $f'$ such that
  $w'_{{\mathrm{1}}} \, w'_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f'$,
  $ \langle   \emptyset    \vdash   \ottsym{(}  w_{{\mathrm{1}}} \, \ottsym{(}  w_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell }  }  \! \ottnt{U_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  \ottnt{f'}  \dashv   \emptyset   \rangle $,
  and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
\end{lemma}
\fi % ifrestate

\begin{proof}
  By \rnp{R\_AppCast},
  $\ottsym{(}  w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \ottsym{)} \, w_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \ottsym{(}  w_{{\mathrm{1}}} \, \ottsym{(}  w_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell }  }  \! \ottnt{U_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{2}}}} $.
  By induction on $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.

  \begin{caseanalysis}
    \case{\rnp{P\_Cast}}
    Here, by Lemma \ref{lem:canonical_forms},
    there exist $w'_{{\mathrm{11}}}$, $\ottnt{U'_{{\mathrm{11}}}}$, $\ottnt{U'_{{\mathrm{12}}}}$, and $\ell'$ such that
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}   \dashv   \emptyset   \rangle $
    and $w'_{{\mathrm{1}}}  \ottsym{=}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.

    By inversion,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
    and $ \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}} $.
    By Lemma \ref{lem:term_prec_to_type_prec},
    $ \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{11}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}} $ and $ \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{12}}}} $.

    By \rnp{R\_AppCast},
    $\ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}   \ottsym{)} \, w'_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \ottsym{(}  w'_{{\mathrm{11}}} \, \ottsym{(}  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{2}}}} $.

    We finish by \rnp{P\_Cast}, \rnp{P\_App}, and \rnp{P\_Cast}.

    \case{\rnp{P\_CastL}}
    Here,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.

    By inversion,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $
    and $ \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}} $.
    By Lemma \ref{lem:term_prec_to_type_prec},
    $ \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{11}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $ and $ \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}} $.

    We finish by \rnp{P\_CastL}, \rnp{P\_App}, and \rnp{P\_CastL}.

    \case{\rnp{P\_CastR}}
    Here, by Lemma \ref{lem:canonical_forms},
    there exist $w'_{{\mathrm{11}}}$, $\ottnt{U'_{{\mathrm{11}}}}$, $\ottnt{U'_{{\mathrm{12}}}}$, and $\ell'$ such that
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}   \dashv   \emptyset   \rangle $
    and $w'_{{\mathrm{1}}}  \ottsym{=}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.

    By inversion,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
    and $ \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}} $.
    By Lemma \ref{lem:term_prec_to_type_prec},
    $ \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} $.
    By inversion, $ \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}} $ and $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{12}}}} $.

    By \rnp{R\_AppCast},
    $\ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}   \ottsym{)} \, w'_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \ottsym{(}  w'_{{\mathrm{11}}} \, \ottsym{(}  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{2}}}} $.

    By \rnp{P\_CastR},
    $ \langle   \emptyset    \vdash   w_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  :  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \dashv   \emptyset   \rangle $.
    %
    By Lemma \ref{lem:prec_catch_up_left_value},
    there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{2}}}$, and $w''_{{\mathrm{2}}}$ such that
    $w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w''_{{\mathrm{2}}}$,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \ottsym{)}  :  w''_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    %
    By Lemma \ref{lem:right_subst_preserve_prec},
    $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $ and
    $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}  :  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
    %
    So,
    $\ottsym{(}  w'_{{\mathrm{11}}} \, \ottsym{(}  w'_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell' }  }  \! \ottnt{U'_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U'_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'_{{\mathrm{2}}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{2}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, \ottsym{(}  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w''_{{\mathrm{2}}}  \ottsym{)}  \ottsym{:}   S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $.

    By the IH,
    there exist $S''_{{\mathrm{0}}}$, $S'_{{\mathrm{3}}}$, and $f''$ such that
    $S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w''_{{\mathrm{2}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{3}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f''$,
    $ \langle   \emptyset    \vdash   \ottsym{(}  w_{{\mathrm{1}}} \, \ottsym{(}  w_{{\mathrm{2}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ {  \bar{ \ell }  }  \! \ottnt{U_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{2}}}}   :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)}  :  f''  \dashv   \emptyset   \rangle $,
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{3}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    So,
    $\ottsym{(}  S'_{{\mathrm{2}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w''_{{\mathrm{2}}}  \ottsym{)}  \ottsym{:}   S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'_{{\mathrm{2}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{3}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f''  \ottsym{:}    S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{12}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \!  S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $
    and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ     S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{3}}}   \circ  S'_{{\mathrm{2}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
    % FIXME: the above is informal?
    % but it seems to be OK

    By Lemma \ref{lem:right_subst_preserve_prec},
    $ \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'_{{\mathrm{3}}}  \circ  S'_{{\mathrm{2}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)} $.
    We finish by \rnp{P\_CastR}.
    \qedhere
  \end{caseanalysis}
\end{proof}

\ifrestate
\lemTermPrecSimulation*
\else
\begin{lemma}[Simulation of More Precise Programs] \label{lem:term_prec_simulation}
  If $ \langle   \emptyset    \vdash   f_{{\mathrm{1}}}  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $ and $f_{{\mathrm{1}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f_{{\mathrm{2}}}$,
  then there exists $S'$, $S'_{{\mathrm{0}}}$, and $f'_{{\mathrm{2}}}$ such that
  $f'_{{\mathrm{1}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f'_{{\mathrm{2}}}$,
  $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{   S'_{{\mathrm{0}}}  \circ  S   \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  f'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
  and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ    S  \circ  S_{{\mathrm{0}}}   \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
\end{lemma}
\fi %ifrestate

\begin{proof}
  By induction on the term precision derivation.

  \begin{caseanalysis}
    \case{\rnp{P\_Op}}
    We are given $f_{{\mathrm{1}}}  \ottsym{=}  \mathit{op} \, \ottsym{(}  f_{{\mathrm{11}}}  \ottsym{,}  f_{{\mathrm{12}}}  \ottsym{)}$ and $f'_{{\mathrm{1}}}  \ottsym{=}  \mathit{op} \, \ottsym{(}  f'_{{\mathrm{11}}}  \ottsym{,}  f'_{{\mathrm{12}}}  \ottsym{)}$
    for some $ \mathit{op} $, $f_{{\mathrm{11}}}$, $f_{{\mathrm{12}}}$, $f'_{{\mathrm{11}}}$, and $f'_{{\mathrm{12}}}$.

    By inversion,
    there exist $\iota_{{\mathrm{1}}}$, $\iota_{{\mathrm{2}}}$, and $\iota$ such that
    $ \mathit{ty} ( \mathit{op} )   \ottsym{=}  \iota_{{\mathrm{1}}}  \!\rightarrow\!  \iota_{{\mathrm{2}}}  \!\rightarrow\!  \iota$.
    $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \iota_{{\mathrm{1}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \iota_{{\mathrm{1}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $ and
    $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \iota_{{\mathrm{2}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \iota_{{\mathrm{2}}}  :  f'_{{\mathrm{12}}}  \dashv   \emptyset   \rangle $
    where $\ottnt{U}  \ottsym{=}  \ottnt{U'} = \iota$.

    By case analysis on the evaluation rule applied to $f_{{\mathrm{1}}}$.

    \begin{caseanalysis}
      \case{\rnp{E\_Step}}
      There exist $\ottnt{E}$ and $f_{{\mathrm{13}}}$ such that $\ottnt{E}  [  f_{{\mathrm{13}}}  ] \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  \ottnt{E}  [  f'_{{\mathrm{13}}}  ]  \ottsym{)}$.
      By inversion, $f_{{\mathrm{13}}} \,  \xrightarrow{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{13}}}$.
      By case analysis on the structure of $\ottnt{E}$.

      \begin{caseanalysis}
        \case{$\ottnt{E}  \ottsym{=}  \left[ \, \right]$}
        Here, $\mathit{op} \, \ottsym{(}  f_{{\mathrm{11}}}  \ottsym{,}  f_{{\mathrm{12}}}  \ottsym{)}  \ottsym{=}  f_{{\mathrm{13}}}$.
        By case analysis on the reduction rule applied to $f_{{\mathrm{13}}}$.

        \begin{caseanalysis}
          \case{\rnp{R\_Op}}
          $f_{{\mathrm{11}}}$ and $f_{{\mathrm{12}}}$ are values.

          By Lemma \ref{lem:prec_catch_up_left_value},
          there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{11}}}$, and $w'_{{\mathrm{11}}}$ such that
          $f'_{{\mathrm{11}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{11}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{11}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \iota_{{\mathrm{1}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{11}}}  \ottsym{(}  \iota_{{\mathrm{1}}}  \ottsym{)}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $\mathit{op} \, \ottsym{(}  f'_{{\mathrm{11}}}  \ottsym{,}  f'_{{\mathrm{12}}}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{11}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, \mathit{op} \, \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{,}  S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}  \ottsym{)}$.

          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \iota_{{\mathrm{2}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{11}}}  \ottsym{(}  \iota_{{\mathrm{2}}}  \ottsym{)}  :  S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By definition,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \iota_{{\mathrm{2}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  \iota_{{\mathrm{2}}}  :  S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:prec_catch_up_left_value},
          there exist $S''_{{\mathrm{0}}}$, $S'_{{\mathrm{12}}}$, and $w'_{{\mathrm{12}}}$ such that
          $S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{12}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{12}}}$.
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \iota_{{\mathrm{2}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{12}}}  \ottsym{(}  \iota_{{\mathrm{2}}}  \ottsym{)}  :  w'_{{\mathrm{12}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{12}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $\mathit{op} \, \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{,}  S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{12}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, \mathit{op} \, \ottsym{(}  S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \ottsym{,}  w'_{{\mathrm{12}}}  \ottsym{)}$.
          By Lemma \ref{lem:term_prec_inversion4},
          there exists $\ottnt{c_{{\mathrm{12}}}}$ such that $c12 = f_{{\mathrm{12}}}  \ottsym{=}  w'_{{\mathrm{12}}}$.

          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \iota_{{\mathrm{1}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  \iota_{{\mathrm{1}}}  :  S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:term_prec_inversion4},
          there exists $\ottnt{c_{{\mathrm{11}}}}$ such that $c11 = f_{{\mathrm{11}}}  \ottsym{=}  S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}$.

          Finally,
          \begin{itemize}
            \item $\mathit{op} \, \ottsym{(}  f'_{{\mathrm{11}}}  \ottsym{,}  f'_{{\mathrm{12}}}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{}  S'_{{\mathrm{12}}}  \circ  S'_{{\mathrm{11}}}  \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \,  \llbracket\mathit{op}\rrbracket ( \ottnt{c_{{\mathrm{11}}}} ,  \ottnt{c_{{\mathrm{12}}}} ) $,
            \item $ \langle   \emptyset    \vdash    \llbracket\mathit{op}\rrbracket ( \ottnt{c_{{\mathrm{11}}}} ,  \ottnt{c_{{\mathrm{12}}}} )   :  \iota   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  \iota  :   \llbracket\mathit{op}\rrbracket ( \ottnt{c_{{\mathrm{11}}}} ,  \ottnt{c_{{\mathrm{12}}}} )   \dashv   \emptyset   \rangle $, and
            \item $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ     S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{12}}}   \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          \end{itemize}

          \otherwise Cannot happen.
        \end{caseanalysis}

        \case{$\ottnt{E}  \ottsym{=}  \mathit{op} \, \ottsym{(}  \ottnt{E'}  \ottsym{,}  \ottnt{f''}  \ottsym{)}$ for some $\ottnt{E'}$ and $\ottnt{f''}$}
        By using the IH.

        \case{$\ottnt{E}  \ottsym{=}  \ottnt{E'} \, \ottnt{f''}$ for some $\ottnt{E'}$ and $\ottnt{f''}$}
        By using the IH.

        \otherwise Cannot happen.
      \end{caseanalysis}
    \end{caseanalysis}

    \case{\rnp{P\_App}}
    We are given $f_{{\mathrm{1}}}  \ottsym{=}  f_{{\mathrm{11}}} \, f_{{\mathrm{12}}}$ and $f'_{{\mathrm{1}}}  \ottsym{=}  f'_{{\mathrm{11}}} \, f'_{{\mathrm{12}}}$
    for some $f_{{\mathrm{11}}}$, $f_{{\mathrm{12}}}$, $f'_{{\mathrm{11}}}$, and $f'_{{\mathrm{12}}}$.

    By inversion,
    $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $ and
    $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{2}}}}  :  f'_{{\mathrm{12}}}  \dashv   \emptyset   \rangle $.

    By case analysis on the evaluation rule applied to $f_{{\mathrm{1}}}$.

    \begin{caseanalysis}
      \case{\rnp{E\_Step}}
      There exist $\ottnt{E}$ and $f_{{\mathrm{13}}}$ such that $\ottnt{E}  [  f_{{\mathrm{13}}}  ] \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  \ottnt{E}  [  f'_{{\mathrm{13}}}  ]  \ottsym{)}$.
      By inversion, $f_{{\mathrm{13}}} \,  \xrightarrow{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{13}}}$.
      By case analysis on the structure of $\ottnt{E}$.

      \begin{caseanalysis}
        \case{$\ottnt{E}  \ottsym{=}  \left[ \, \right]$}
        Here, $f_{{\mathrm{11}}} \, f_{{\mathrm{12}}}  \ottsym{=}  f_{{\mathrm{13}}}$.
        By case analysis on the reduction rule applied to $f_{{\mathrm{13}}}$.

        \begin{caseanalysis}
          \case{\rnp{R\_Beta}}
          There exist $\ottnt{U_{{\mathrm{11}}}}$, $f_{{\mathrm{111}}}$, and $w_{{\mathrm{12}}}$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}   \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{11}}}}  .\,  f_{{\mathrm{111}}} $, $f_{{\mathrm{12}}}  \ottsym{=}  w_{{\mathrm{12}}}$, and $f_{{\mathrm{2}}}  \ottsym{=}  f_{{\mathrm{111}}}  [  \ottmv{x}  \ottsym{:=}  w_{{\mathrm{12}}}  ]$.
          Here, $S  \ottsym{=}  [  ]$.

          By Lemma \ref{lem:prec_catch_up_left_value},
          there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{11}}}$, and $w'_{{\mathrm{11}}}$ such that
          $f'_{{\mathrm{11}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{11}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{11}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{11}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $f'_{{\mathrm{11}}} \, f'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{11}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{11}}} \, S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}$.

          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{11}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:prec_catch_up_left_value},
          there exist $S''_{{\mathrm{0}}}$, $S'_{{\mathrm{12}}}$, and $w'_{{\mathrm{12}}}$ such that
          $S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{12}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{12}}}$.
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{12}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  w'_{{\mathrm{12}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{12}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $w'_{{\mathrm{11}}} \, S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{12}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w'_{{\mathrm{12}}}$.

          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'_{{\mathrm{12}}}  \circ  S'_{{\mathrm{11}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:term_prec_simulation_app},
          there exist $S'''_{{\mathrm{0}}}$, $S'$, and $f'_{{\mathrm{2}}}$ such that
          $S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f'_{{\mathrm{2}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{    S'''_{{\mathrm{0}}}  \circ  S''_{{\mathrm{0}}}   \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'  \circ   S'_{{\mathrm{12}}}  \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  f'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}    S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \ottsym{)}.   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'''_{{\mathrm{0}}}  \circ     S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{2}}}$.

          Finally, $f'_{{\mathrm{11}}} \, f'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{}   S'  \circ  S'_{{\mathrm{12}}}   \circ  S'_{{\mathrm{11}}}  \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f'_{{\mathrm{2}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  \ottnt{U_{{\mathrm{12}}}}   \sqsubseteq _{    S'''_{{\mathrm{0}}}  \circ  S''_{{\mathrm{0}}}   \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'  \circ   S'_{{\mathrm{12}}}  \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  f'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'''_{{\mathrm{0}}}  \circ       S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \circ  S'   \circ  S'_{{\mathrm{12}}}   \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.

          \case{\rnp{R\_AppCast}}
          We are given $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{11}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \! \ottnt{U_{{\mathrm{13}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{14}}}} $, $f_{{\mathrm{12}}}  \ottsym{=}  w_{{\mathrm{12}}}$,
          $f_{{\mathrm{2}}}  \ottsym{=}  \ottsym{(}  w_{{\mathrm{11}}} \, \ottsym{(}  w_{{\mathrm{12}}}  \ottsym{:}   \ottnt{U_{{\mathrm{13}}}} \Rightarrow  \unskip ^ {  \bar{ \ell_{{\mathrm{1}}} }  }  \! \ottnt{U_{{\mathrm{11}}}}   \ottsym{)}  \ottsym{)}  \ottsym{:}   \ottnt{U_{{\mathrm{12}}}} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \! \ottnt{U_{{\mathrm{14}}}} $ for some
          $w_{{\mathrm{11}}}$, $w_{{\mathrm{12}}}$, $\ottnt{U_{{\mathrm{11}}}}$, $\ottnt{U_{{\mathrm{12}}}}$,
          $\ottnt{U_{{\mathrm{13}}}}$, $\ottnt{U_{{\mathrm{14}}}}$, and $\ell_{{\mathrm{1}}}$.
          Here, $S  \ottsym{=}  [  ]$.

          By Lemma \ref{lem:prec_catch_up_left_value},
          there exist $S'_{{\mathrm{0}}}$, $S'_{{\mathrm{11}}}$, and $w'_{{\mathrm{11}}}$ such that
          $f'_{{\mathrm{11}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{11}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{11}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{11}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ   S_{{\mathrm{0}}}  \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $f'_{{\mathrm{11}}} \, f'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{11}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{11}}} \, S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}$.

          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{11}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:prec_catch_up_left_value},
          there exist $S''_{{\mathrm{0}}}$, $S'_{{\mathrm{12}}}$, and $w'_{{\mathrm{12}}}$ such that
          $f'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{12}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'_{{\mathrm{12}}}$.
          $ \langle   \emptyset    \vdash   f_{{\mathrm{12}}}  :  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  S'_{{\mathrm{12}}}  \ottsym{(}  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  w'_{{\mathrm{12}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S''_{{\mathrm{0}}}  \circ    S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}   \circ  S'_{{\mathrm{12}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
          So, $w'_{{\mathrm{11}}} \, S'_{{\mathrm{11}}}  \ottsym{(}  f'_{{\mathrm{12}}}  \ottsym{)} \,  \xmapsto{ \mathmakebox[0.4em]{} S'_{{\mathrm{12}}} \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w'_{{\mathrm{12}}}$.

          By Lemma \ref{lem:right_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}   \sqsubseteq _{   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }   S'_{{\mathrm{12}}}  \circ  S'_{{\mathrm{11}}}   \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}}  \ottsym{)}  :  S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:term_prec_simulation_unwrap},
          there exist $S'''_{{\mathrm{0}}}$, $S'$, and $f'_{{\mathrm{2}}}$ such that
          $S'_{{\mathrm{12}}}  \ottsym{(}  w'_{{\mathrm{11}}}  \ottsym{)} \, w'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f'_{{\mathrm{2}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  \ottnt{U}   \sqsubseteq _{    S'''_{{\mathrm{0}}}  \circ  S''_{{\mathrm{0}}}   \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}    S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \ottsym{)}.   S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'''_{{\mathrm{0}}}  \circ     S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.

          Finally, $f'_{{\mathrm{11}}} \, f'_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{}   S'  \circ  S'_{{\mathrm{12}}}   \circ  S'_{{\mathrm{11}}}  \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, f'_{{\mathrm{2}}}$,
          $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  \ottnt{U}   \sqsubseteq _{    S'''_{{\mathrm{0}}}  \circ  S''_{{\mathrm{0}}}   \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'_{{\mathrm{2}}}  \dashv   \emptyset   \rangle $,
          and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}  S_{{\mathrm{0}}}  \ottsym{)}. S_{{\mathrm{0}}}  \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'''_{{\mathrm{0}}}  \circ       S''_{{\mathrm{0}}}  \circ  S'_{{\mathrm{0}}}   \circ  S_{{\mathrm{0}}}   \circ  S'   \circ  S'_{{\mathrm{12}}}   \circ  S'_{{\mathrm{11}}}    \ottsym{(}  \ottmv{X}  \ottsym{)}$.

          \otherwise Contradictory.
        \end{caseanalysis}

        \case{$\ottnt{E}  \ottsym{=}  \ottnt{E_{{\mathrm{1}}}} \, f_{{\mathrm{12}}}$ for some $\ottnt{E_{{\mathrm{1}}}}$}
        By using the IH.

        \case{$\ottnt{E}  \ottsym{=}  w_{{\mathrm{11}}} \, \ottnt{E_{{\mathrm{1}}}}$ for some $\ottnt{E_{{\mathrm{1}}}}$ and $w_{{\mathrm{11}}}$ where $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$}
        By using the IH.

        \otherwise
        Contradictory.
      \end{caseanalysis}

      \case{\rnp{E\_Abort}}
      Here, $f_{{\mathrm{11}}} \, f_{{\mathrm{12}}} \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \textsf{\textup{blame}\relax} \, \ell$ for some $\ell$.
      We finish by \rnp{P\_Blame}.
    \end{caseanalysis}

    % \case{\rnp{P\_LetP}}
    % Obviously by using Lemma \ref{lem:subst_preserve_term_prec}.
    %
    % % There exists $\ottmv{x}$, $ \overrightarrow{ \ottmv{X_{\ottmv{i}}} } $, $ \overrightarrow{ \ottmv{X'_{\ottmv{i}}} } $, $w_{{\mathrm{1}}}$, $w'_{{\mathrm{1}}}$,
    % % $f_{{\mathrm{11}}}$, and $f'_{{\mathrm{11}}}$ such that
    % % $f_{{\mathrm{1}}}  \ottsym{=}   \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{1}}}   \textsf{\textup{ in }\relax}  f_{{\mathrm{11}}} $ and
    % % $f'_{{\mathrm{1}}}  \ottsym{=}   \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{1}}}   \textsf{\textup{ in }\relax}  f'_{{\mathrm{11}}} $.
    % % By inversion,
    % % $ \langle   \emptyset    \vdash   w_{{\mathrm{1}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  w'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $,
    % % $ \langle   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{11}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  :  f'_{{\mathrm{11}}}  \dashv   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}   \rangle $,
    % % $ \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \cap  \textit{ftv} \, \ottsym{(}  \Gamma  \ottsym{)}  \ottsym{=}   \emptyset $ and $ \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \cap  \textit{ftv} \, \ottsym{(}  \Gamma'  \ottsym{)}  \ottsym{=}   \emptyset $.
    % %
    % % By definition,
    % % $ \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{1}}}   \textsf{\textup{ in }\relax}  f_{{\mathrm{11}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, f_{{\mathrm{11}}}  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{1}}}   ]$ and
    % % $ \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{1}}}   \textsf{\textup{ in }\relax}  f'_{{\mathrm{11}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{11}}}  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{1}}}   ]$.
    % %
    % % By Lemma \ref{lem:subst_preserve_term_prec},
    % % $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{1}}}   ]  :  \ottnt{U_{{\mathrm{11}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{11}}}}  :  f'_{{\mathrm{11}}}  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{1}}}   ]  \dashv   \emptyset   \rangle $.

    \case{\rnp{P\_LetP}}
    We are given $f_{{\mathrm{1}}}  \ottsym{=}   \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{11}}}   \textsf{\textup{ in }\relax}  f_{{\mathrm{12}}} $ and
    $f'_{{\mathrm{1}}}  \ottsym{=}   \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{11}}}   \textsf{\textup{ in }\relax}  f'_{{\mathrm{12}}} $
    for some $ \overrightarrow{ \ottmv{X_{\ottmv{i}}} } $, $ \overrightarrow{ \ottmv{X'_{\ottmv{i}}} } $, $w_{{\mathrm{11}}}$, $w'_{{\mathrm{11}}}$,
    $f_{{\mathrm{12}}}$, and $f'_{{\mathrm{12}}}$.
    By inversion,
    $ \langle   \emptyset    \vdash   w_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  w'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $, and
    $ \langle   \ottmv{x}  :  \forall \,  \overrightarrow{ \ottmv{X_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U_{{\mathrm{1}}}}    \vdash   f_{{\mathrm{12}}}  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{12}}}  \dashv   \ottmv{x'}  :  \forall \,  \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }   \ottsym{.}  \ottnt{U'_{{\mathrm{1}}}}   \rangle $.
    By case analysis on the evaluation rule applied to $f_{{\mathrm{1}}}$.

    \begin{caseanalysis}
      \case{\rnp{E\_Step}}
      There exists $\ottnt{E}$ and $f_{{\mathrm{13}}}$ such that $\ottnt{E}  [  f_{{\mathrm{13}}}  ] \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  \ottnt{E}  [  f'_{{\mathrm{13}}}  ]  \ottsym{)}$.
      By inversion, $f_{{\mathrm{13}}} \,  \xrightarrow{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{13}}}$.
      By case analysis on the structure of $\ottnt{E}$.

      \begin{caseanalysis}
        \case{$\ottnt{E}  \ottsym{=}  \left[ \, \right]$}
        Here, $f_{{\mathrm{1}}}  \ottsym{=}  f_{{\mathrm{13}}}$.
        By case analysis on the reduction rule applied to $f_{{\mathrm{13}}}$.

        \begin{caseanalysis}
          \case{\rnp{R\_LetP}}
          We are given $ \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{11}}}   \textsf{\textup{ in }\relax}  f_{{\mathrm{12}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, f_{{\mathrm{12}}}  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X_{\ottmv{i}}} }  .\,  w_{{\mathrm{11}}}   ]$.

          By \rnp{R\_LetP},
          $ \textsf{\textup{let}\relax} \,  \ottmv{x}  =   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{11}}}   \textsf{\textup{ in }\relax}  f'_{{\mathrm{12}}}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{12}}}  [  \ottmv{x}  \ottsym{:=}   \Lambda    \overrightarrow{ \ottmv{X'_{\ottmv{i}}} }  .\,  w'_{{\mathrm{11}}}   ]$.

          We finish by Lemma \ref{lem:subst_preserve_term_prec}.

          \otherwise Cannot happen.
        \end{caseanalysis}

        \otherwise Cannot happen.
      \end{caseanalysis}

      \case{\rnp{E\_Abort}}
      Cannot happen.
    \end{caseanalysis}

    \case{\rnp{P\_Cast}}
    We are given $f_{{\mathrm{1}}}  \ottsym{=}  f_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U} $ and $f'_{{\mathrm{1}}}  \ottsym{=}  f'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'} $
    for some $f_{{\mathrm{11}}}$, $f'_{{\mathrm{11}}}$, $\ottnt{U_{{\mathrm{1}}}}$, $\ottnt{U'_{{\mathrm{1}}}}$, $\ell$, and $\ell'$.

    By inversion,
    $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $,
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $, $\ottnt{U_{{\mathrm{1}}}}  \sim  \ottnt{U}$, and $\ottnt{U'_{{\mathrm{1}}}}  \sim  \ottnt{U'}$.

    By case analysis on the evaluation rule applied to $f_{{\mathrm{1}}}$.

    \begin{caseanalysis}
      \case{\rnp{E\_Step}}
      There exist $\ottnt{E}$ and $f_{{\mathrm{12}}}$ such that $\ottnt{E}  [  f_{{\mathrm{12}}}  ] \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  \ottnt{E}  [  f'_{{\mathrm{12}}}  ]  \ottsym{)}$.
      By inversion, $f_{{\mathrm{12}}} \,  \xrightarrow{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{12}}}$.
      By case analysis on the structure of $\ottnt{E}$.

      \begin{caseanalysis}
        \case{$\ottnt{E}  \ottsym{=}  \left[ \, \right]$}
        Here, $f_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}   \ottsym{=}  f_{{\mathrm{12}}}$.
        By case analysis on the reduction rule applied to $f_{{\mathrm{12}}}$.

        \begin{caseanalysis}
          \case{\rnp{R\_IdBase}}
          There exist $w_{{\mathrm{11}}}$ and $\iota$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \iota$ and $\ottnt{U}  \ottsym{=}  \iota$.
          $w_{{\mathrm{11}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell }  \! \iota  \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, w_{{\mathrm{11}}}$ where $S  \ottsym{=}  [  ]$.
          By Lemma \ref{lem:term_prec_to_type_prec},
          $ \iota   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
          By \rnp{P\_CastR},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{11}}}  :  \iota   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}   \dashv   \emptyset   \rangle $.

          \case{\rnp{R\_IdStar}}
          Similarly to the case \rnp{R\_IdBase}.

          \case{\rnp{R\_Succeed}}
          There exist $w_{{\mathrm{111}}}$ and $\ottnt{G}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$ and $\ottnt{U}  \ottsym{=}  \ottnt{G}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}   \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, w_{{\mathrm{111}}}$ where $S  \ottsym{=}  [  ]$.
          Here, $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \! \star   :  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:term_prec_inversion3},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  :  \ottnt{G}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:term_prec_to_type_prec},
          $ \ottnt{G}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
          By \rnp{P\_CastR},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  :  \ottnt{G}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}   \dashv   \emptyset   \rangle $.

          \case{\rnp{R\_Fail}}
          There exist $w_{{\mathrm{111}}}$, $\ottnt{G}$, $\ottnt{G'}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$ and $\ottnt{U}  \ottsym{=}  \ottnt{G}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}   \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, \textsf{\textup{blame}\relax} \, \ell$ where $S  \ottsym{=}  [  ]$.
          We finish by \rnp{P\_Blame}.

          \case{\rnp{R\_Ground}}
          There exist $w_{{\mathrm{11}}}$ and $\ottnt{G}$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$, $\ottnt{U}  \ottsym{=}  \star$, and $\ottnt{U_{{\mathrm{1}}}}  \sim  \ottnt{G}$.
          $w_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \star  \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, w_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \!  \ottnt{G} \Rightarrow  \unskip ^ { \ell }  \! \star  $ where $S  \ottsym{=}  [  ]$.
          We finish by \rnp{P\_Cast} and \rnp{P\_CastL}.

          \case{\rnp{R\_Expand}}
          There exist $w_{{\mathrm{11}}}$ and $\ottnt{G}$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$, and $\ottnt{U}  \sim  \ottnt{G}$.
          $w_{{\mathrm{11}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}  \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, w_{{\mathrm{11}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell }  \!  \ottnt{G} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}  $ where $S  \ottsym{=}  [  ]$.
          We finish by \rnp{P\_CastL} and \rnp{P\_Cast}.

          \case{\rnp{R\_InstBase}}
          There exist $w_{{\mathrm{111}}}$, $\iota$, and $\ottmv{X}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$, and $\ottnt{U}  \ottsym{=}  \ottmv{X}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}   \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}$ where $S  \ottsym{=}  [  \ottmv{X}  :=  \iota  ]$.
          By Lemma \ref{lem:term_prec_inversion3},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  :  \iota   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.
          %
          By Lemma \ref{lem:left_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  :  \iota   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
          and $ S  \ottsym{(}  \ottmv{X}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
          So, $ \iota   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
          %
          By \rnp{P\_CastR},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  :  \iota   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}   \dashv   \emptyset   \rangle $

          \case{\rnp{R\_InstArrow}}
          There exist $w_{{\mathrm{111}}}$ and $\ottmv{X}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$ and $\ottnt{U}  \ottsym{=}  \ottmv{X}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}   \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}   $
          where $S  \ottsym{=}  [  \ottmv{X}  :=  \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}  ]$.
          %
          By Lemma \ref{lem:term_prec_to_type_prec},
          $ \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}} $.
          By definition, $\ottnt{U'_{{\mathrm{1}}}}  \ottsym{=}  \star$.
          %
          Here, $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \! \star   :  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \star  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
          and $ \ottmv{X}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
          %
          By \rnp{P\_CastL},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \star  \!\rightarrow\!  \star    :  \star  \!\rightarrow\!  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \star  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $.
          %
          By Lemma \ref{lem:left_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \star  \!\rightarrow\!  \star    :  \star  \!\rightarrow\!  \star   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \star  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $
          and $ S  \ottsym{(}  \ottmv{X}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
          So, $ \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
          %
          By \rnp{P\_Cast},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}     :  \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'_{{\mathrm{11}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}   \dashv   \emptyset   \rangle $.

          \otherwise
          Contradictory.
        \end{caseanalysis}

        \case{$\ottnt{E}  \ottsym{=}  \ottnt{E_{{\mathrm{1}}}}  \ottsym{:}  \ottnt{U_{{\mathrm{1}}}}  \Rightarrow   \unskip ^ { \ell }  \, \ottnt{U}$ for some $\ottnt{E_{{\mathrm{1}}}}$}
        By using the IH.

        \otherwise
        Contradictory.
      \end{caseanalysis}

      \case{\rnp{E\_Abort}}
      Here, $f_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \textsf{\textup{blame}\relax} \, \ell_{{\mathrm{1}}}$ for some $\ell_{{\mathrm{1}}}$.
      We finish by \rnp{P\_Blame}.
    \end{caseanalysis}

    \case{\rnp{P\_CastL}}
    We are given $f_{{\mathrm{1}}}  \ottsym{=}  f_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U} $
    for some $f_{{\mathrm{11}}}$, $\ottnt{U_{{\mathrm{1}}}}$, and $\ell$.

    By inversion,
    $ \langle   \emptyset    \vdash   f_{{\mathrm{11}}}  :  \ottnt{U_{{\mathrm{1}}}}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $,
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $, and $\ottnt{U_{{\mathrm{1}}}}  \sim  \ottnt{U}$.

    By case analysis on the evaluation rule applied to $f_{{\mathrm{1}}}$.

    \begin{caseanalysis}
      \case{\rnp{E\_Step}}
      There exist $\ottnt{E}$ and $f_{{\mathrm{12}}}$ such that $\ottnt{E}  [  f_{{\mathrm{12}}}  ] \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  \ottnt{E}  [  f'_{{\mathrm{12}}}  ]  \ottsym{)}$.
      By inversion, $f_{{\mathrm{12}}} \,  \xrightarrow{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{12}}}$.
      By case analysis on the structure of $\ottnt{E}$.

      \begin{caseanalysis}
        \case{$\ottnt{E}  \ottsym{=}  \left[ \, \right]$}
        Here, $f_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}   \ottsym{=}  f_{{\mathrm{12}}}$.
        By case analysis on the reduction rule applied to $f_{{\mathrm{12}}}$.

        \begin{caseanalysis}
          \case{\rnp{R\_IdBase}}
          There exist $w_{{\mathrm{11}}}$ and $\iota$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \iota$ and $\ottnt{U}  \ottsym{=}  \iota$.
          $w_{{\mathrm{11}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell }  \! \iota  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w_{{\mathrm{11}}}$.

          \case{\rnp{R\_IdStar}}
          Similarly to the case \rnp{R\_IdBase}.

          \case{\rnp{R\_Succeed}}
          There exist $w_{{\mathrm{111}}}$ and $\ottnt{G}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$ and $\ottnt{U}  \ottsym{=}  \ottnt{G}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}   \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w_{{\mathrm{111}}}$.
          Here, $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \! \star   :  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:term_prec_inversion3},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  :  \ottnt{G}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.

          \case{\rnp{R\_Fail}}
          There exist $w_{{\mathrm{111}}}$, $\ottnt{G}$, $\ottnt{G'}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$ and $\ottnt{U}  \ottsym{=}  \ottnt{G}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \ottnt{G'} \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{G}   \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \textsf{\textup{blame}\relax} \, \ell$.
          We finish by \rnp{P\_Blame}.

          \case{\rnp{R\_Ground}}
          There exist $w_{{\mathrm{11}}}$ and $\ottnt{G}$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$, $\ottnt{U}  \ottsym{=}  \star$, and $\ottnt{U_{{\mathrm{1}}}}  \sim  \ottnt{G}$.
          $w_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \star  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \!  \ottnt{G} \Rightarrow  \unskip ^ { \ell }  \! \star  $.
          We finish by \rnp{P\_CastL}.

          \case{\rnp{R\_Expand}}
          There exist $w_{{\mathrm{11}}}$ and $\ottnt{G}$ such that
          $f_{{\mathrm{11}}}  \ottsym{=}  w_{{\mathrm{11}}}$, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$, and $\ottnt{U}  \sim  \ottnt{G}$.
          $w_{{\mathrm{11}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, w_{{\mathrm{11}}}  \ottsym{:}   \star \Rightarrow  \unskip ^ { \ell }  \!  \ottnt{G} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}  $.
          We finish by \rnp{P\_CastL}.

          \case{\rnp{R\_InstBase}}
          There exist $w_{{\mathrm{111}}}$, $\iota$, and $\ottmv{X}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$, and $\ottnt{U}  \ottsym{=}  \ottmv{X}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \iota \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}   \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}$ where $S  \ottsym{=}  [  \ottmv{X}  :=  \iota  ]$.
          By Lemma \ref{lem:term_prec_inversion3},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  :  \iota   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.
          By Lemma \ref{lem:left_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  :  \iota   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'}  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $

          \case{\rnp{R\_InstArrow}}
          There exist $w_{{\mathrm{111}}}$ and $\ottmv{X}$ such that
          $f_{{\mathrm{1}}}  \ottsym{=}  w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}  $, $\ottnt{U_{{\mathrm{1}}}}  \ottsym{=}  \star$ and $\ottnt{U}  \ottsym{=}  \ottmv{X}$.
          $w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X}   \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}   $
          where $S  \ottsym{=}  [  \ottmv{X}  :=  \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}  ]$.
          %
          By Lemma \ref{lem:term_prec_to_type_prec},
          $ \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
          By definition, $\ottnt{U'}  \ottsym{=}  \star$.
          %
          Here, $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \! \star   :  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \star  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.
          %
          By \rnp{P\_CastL},
          $ \langle   \emptyset    \vdash   w_{{\mathrm{111}}}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \star  \!\rightarrow\!  \star    :  \star  \!\rightarrow\!  \star   \sqsubseteq _{ S_{{\mathrm{0}}} }  \star  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.
          %
          By Lemma \ref{lem:left_subst_preserve_prec},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \! \star  \!\rightarrow\!  \star    :  \star  \!\rightarrow\!  \star   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \star  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $
          and $ S  \ottsym{(}  \ottmv{X}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
          So, $ \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
          %
          By \rnp{P\_CastL},
          $ \langle   \emptyset    \vdash   S  \ottsym{(}  w_{{\mathrm{111}}}  \ottsym{)}  \ottsym{:}   \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell_{{\mathrm{1}}} }  \!  \star \Rightarrow  \unskip ^ { \ell }  \!  \star  \!\rightarrow\!  \star \Rightarrow  \unskip ^ { \ell }  \! \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}     :  \ottmv{X_{{\mathrm{1}}}}  \!\rightarrow\!  \ottmv{X_{{\mathrm{2}}}}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \star  :  f'_{{\mathrm{1}}}  \dashv   \emptyset   \rangle $.

          \otherwise
          Contradictory.
        \end{caseanalysis}

        \case{$\ottnt{E}  \ottsym{=}  \ottnt{E_{{\mathrm{1}}}}  \ottsym{:}  \ottnt{U_{{\mathrm{1}}}}  \Rightarrow   \unskip ^ { \ell }  \, \ottnt{U}$ for some $\ottnt{E_{{\mathrm{1}}}}$}
        By using the IH.

        \otherwise
        Contradictory.
      \end{caseanalysis}

      \case{\rnp{E\_Abort}}
      Here, $f_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U}  \,  \xmapsto{ \mathmakebox[0.4em]{} [  ] \mathmakebox[0.3em]{} }  \, \textsf{\textup{blame}\relax} \, \ell_{{\mathrm{1}}}$ for some $\ell_{{\mathrm{1}}}$.
      We finish by \rnp{P\_Blame}.
    \end{caseanalysis}

    \case{\rnp{P\_CastR}}
    We are given $f'_{{\mathrm{1}}}  \ottsym{=}  f'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'} $
    for some $f'_{{\mathrm{11}}}$, $\ottnt{U'_{{\mathrm{1}}}}$, and $\ell'$.
    %
    By inversion,
    $ \langle   \emptyset    \vdash   f_{{\mathrm{1}}}  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'_{{\mathrm{1}}}}  :  f'_{{\mathrm{11}}}  \dashv   \emptyset   \rangle $,
    $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $, and $\ottnt{U'_{{\mathrm{1}}}}  \sim  \ottnt{U'}$.

    By case analysis on the evaluation rule applied to $f_{{\mathrm{1}}}$.

    \begin{caseanalysis}
      \case{\rnp{E\_Step}}
      There exist $\ottnt{E}$ and $f_{{\mathrm{12}}}$ such that $\ottnt{E}  [  f_{{\mathrm{12}}}  ] \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, S  \ottsym{(}  \ottnt{E}  [  f'_{{\mathrm{12}}}  ]  \ottsym{)}$.
      By inversion, $f_{{\mathrm{12}}} \,  \xrightarrow{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{12}}}$.
      By case analysis on the structure of $\ottnt{E}$.

      \begin{caseanalysis}
        \case{$\ottnt{E}  \ottsym{=}  \left[ \, \right]$}
        We are given $f_{{\mathrm{1}}}  \ottsym{=}  f_{{\mathrm{12}}}$.

        By the IH, there exist $S'_{{\mathrm{0}}}$, $S'$, and $f'_{{\mathrm{21}}}$
        such that $f'_{{\mathrm{11}}} \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{21}}}$,
        $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{   S'_{{\mathrm{0}}}  \circ  S   \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)}  :  f'_{{\mathrm{21}}}  \dashv   \emptyset   \rangle $,
        and $\forall \ottmv{X} \in \textit{dom} \, \ottsym{(}   S  \circ  S_{{\mathrm{0}}}   \ottsym{)}.  S  \circ  S_{{\mathrm{0}}}   \ottsym{(}  \ottmv{X}  \ottsym{)}  \ottsym{=}   S'_{{\mathrm{0}}}  \circ    S  \circ  S_{{\mathrm{0}}}   \circ  S'    \ottsym{(}  \ottmv{X}  \ottsym{)}$.
        So, $f'_{{\mathrm{11}}}  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}} \Rightarrow  \unskip ^ { \ell' }  \! \ottnt{U'}  \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }  \, f'_{{\mathrm{21}}}  \ottsym{:}   S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'  \ottsym{(}  \ottnt{U'}  \ottsym{)} $.

        By Lemma \ref{lem:left_subst_preserve_prec},
        $ S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{  S  \circ  S_{{\mathrm{0}}}  }  \ottnt{U'} $.
        By Lemma \ref{lem:right_subst_preserve_prec},
        $ S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{   S'_{{\mathrm{0}}}  \circ  S   \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)} $.

        By \rnp{P\_CastR},
        $ \langle   \emptyset    \vdash   f_{{\mathrm{2}}}  :  S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{   S'_{{\mathrm{0}}}  \circ  S   \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  f'_{{\mathrm{21}}}  \ottsym{:}   S'  \ottsym{(}  \ottnt{U'_{{\mathrm{1}}}}  \ottsym{)} \Rightarrow  \unskip ^ { \ell' }  \! S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}   \dashv   \emptyset   \rangle $.

        \otherwise
        By using the IH.
      \end{caseanalysis}
    \end{caseanalysis}

    \otherwise Cannot happen.  \qedhere
  \end{caseanalysis}
\end{proof}

% \subsection{Gradual Guarantee}

\ifrestate
\thmGg*
\else
\begin{theorem}[Gradual Guarantee] \label{thm:gg}
  Suppose $ \langle   \emptyset    \vdash   f  :  \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'}  :  f'  \dashv   \emptyset   \rangle $ and $ \emptyset   \vdash  f  \ottsym{:}  \ottnt{U}$.

  \begin{enumerate}
    \item $ \emptyset   \vdash  f'  \ottsym{:}  \ottnt{U'}$ and $ \ottnt{U}   \sqsubseteq _{ S_{{\mathrm{0}}} }  \ottnt{U'} $.
    \item
      \begin{itemize}
        \item If $f \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w$,
          then there exist $w'$ and $S'_{{\mathrm{0}}}$ such that
          $f' \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'$ and
          $ \langle   \emptyset    \vdash   w  :  S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  w'  \dashv   \emptyset   \rangle $.
        \item If $ f \!  \Uparrow  $, then $ f' \!  \Uparrow  $.
      \end{itemize}
    \item
      \begin{itemize}
        \item If $f' \,  \xmapsto{ \mathmakebox[0.4em]{} S' \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, w'$,
          then there exist $w$ and $S'_{{\mathrm{0}}}$ such that
          $ \langle   \emptyset    \vdash   w  :  S  \ottsym{(}  \ottnt{U}  \ottsym{)}   \sqsubseteq _{  S'_{{\mathrm{0}}}  \circ  S_{{\mathrm{0}}}  }  S'  \ottsym{(}  \ottnt{U'}  \ottsym{)}  :  w'  \dashv   \emptyset   \rangle $,
          or there exists $\ell$ such that $f \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, \textsf{\textup{blame}\relax} \, \ell$.
        \item If $ f' \!  \Uparrow  $,
          then $ f \!  \Uparrow  $
          or there exists $\ell$ such that $f \,  \xmapsto{ \mathmakebox[0.4em]{} S \mathmakebox[0.3em]{} }\hspace{-0.4em}{}^\ast \hspace{0.2em}  \, \textsf{\textup{blame}\relax} \, \ell$.
      \end{itemize}
  \end{enumerate}
\end{theorem}
\fi %ifrestate

\begin{proof}
  \leavevmode
  \begin{enumerate}
    \item By Lemmas \ref{lem:term_prec_to_type_prec} and \ref{lem:term_prec_to_typing}.
    \item
      \begin{itemize}
        \item
          By induction on the evaluation sequence using
          Lemmas \ref{lem:prec_catch_up_left_value} and \ref{lem:term_prec_simulation}.
        \item
          Here, there is an infinite evaluation sequence from $f$,
          and it contains infinite times application of \rnp{R\_Beta}.
          By Lemma \ref{lem:term_prec_simulation_app},
          there is an infinite evaluation sequence from $f'$.
          % \fixme{informal, is it OK?}
      \end{itemize}
    \item
      \begin{itemize}
        \item By contradiction using Theorem \ref{thm:gg}.2.
        \item By contradiction using Theorem \ref{thm:gg}.2.  \qedhere
      \end{itemize}
  \end{enumerate}
\end{proof}

\end{document}


==> sections/acknowledgments.tex <==
% vim: spell
\acknowledgments
First of all, I would like to thank my supervisor, Prof.~Atsushi Igarashi, for
giving me a chance to study gradual typing.  He also gave me many essential and
faithful comments through discussions.  I could not finish my master's course
without his continuous support.

I also thank Prof.~Kohei Suenaga and Prof.~Seiji Umatani for helpful comments
at the laboratory seminars.  They also give me good advice on my presentations.

I thank Prof.~Susumu Nishimura, at Graduate School of Science, for reviewing
this master's thesis.

I thank Dr.~Taro Sekiyama for introducing me to the research
field and giving me useful comments.

I am grateful to all members of the laboratory for both discussions and daily
small talks.  In particular, I thank Mr.~Yuu Igarashi for everyday discussions.  I
could learn a lot from them.

Lastly, I thank my family for both financial and mental support.


==> sections/cast_insertion.tex <==
\section{Cast Insertion} \label{sec:cast_insertion}
\input{figures/def_cast_insertion}


==> sections/proofs.tex <==
\section{Proofs of Properties} \label{sec:proofs}

\subsection{Type Safety}
\input{proofs/type_progress}
\input{proofs/type_preservation}
\input{proofs/type_safety}

\subsection{Soundness of Dynamic Type Inference}
\input{proofs/soundness}

\subsection{Divergence}
\input{proofs/divergence}

\subsection{Completeness of Dynamic Type Inference}
\input{proofs/completeness}

\subsection{The Gradual Guarantee}
\input{proofs/gg}


==> sections/statements.tex <==
\begin{restatable}[Canonical Forms]{lemma}{lemCanonicalForms} \label{lem:canonical_forms}
  If $ \emptyset   \vdash  w  \ottsym{:}  \ottnt{U}$, then one of the following holds:
  \begin{itemize}
    \item $\ottnt{U}  \ottsym{=}  \iota$ and $w  \ottsym{=}  \ottnt{c}$ for some $\ottnt{c}$;
    \item $\ottnt{U}  \ottsym{=}  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}$ and $w  \ottsym{=}   \lambda  \ottmv{x} \!:\!  \ottnt{U_{{\mathrm{1}}}}  .\,  \ottnt{f} $ for some $\ottmv{x}$, $\ottnt{f}$, $\ottnt{U_{{\mathrm{1}}}}$, and $\ottnt{U_{{\mathrm{2}}}}$;
    \item $\ottnt{U}  \ottsym{=}  \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}}$ and $w  \ottsym{=}  w'  \ottsym{:}   \ottnt{U'_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U'_{{\mathrm{2}}}} \Rightarrow  \unskip ^ { \ell }  \! \ottnt{U_{{\mathrm{1}}}}  \!\rightarrow\!  \ottnt{U_{{\mathrm{2}}}} $
      for some $w'$, $\ottnt{U_{{\mathrm{1}}}}, \ottnt{U_{{\mathrm{2}}}}, \ottnt{U'_{{\mathrm{1}}}}$, and $\ottnt{U'_{{\mathrm{2}}}}$; or
    \item $\ottnt{U}  \ottsym{=}  \star$ and $w  \ottsym{=}  w'  \ottsym{:}   \ottnt{G} \Rightarrow  \unskip ^ { \ell }  \! \star $
      for some $w'$, $\ottnt{G}$, and $\ell$.
  \end{itemize}
\end{restatable}

